An Expectation-Based Network Scan Statistic for a COVID-19 Early Warning System

One of the Greater London Authority's (GLA) response to the COVID-19 pandemic brings together multiple large-scale and heterogeneous datasets capturing mobility, transportation and traffic activity over the city of London to better understand 'busyness' and enable targeted interventions and effective policy-making. As part of Project Odysseus we describe an early-warning system and introduce an expectation-based scan statistic for networks to help the GLA and Transport for London, understand the extent to which populations are following government COVID-19 guidelines. We explicitly treat the case of geographically fixed time-series data located on a (road) network and primarily focus on monitoring the dynamics across large regions of the capital. Additionally, we also focus on the detection and reporting of significant spatio-temporal regions. Our approach is extending the Network Based Scan Statistic (NBSS) by making it expectation-based (EBP) and by using stochastic processes for time-series forecasting, which enables us to quantify metric uncertainty in both the EBP and NBSS frameworks. We introduce a variant of the metric used in the EBP model which focuses on identifying space-time regions in which activity is quieter than expected.

==> sections/discussion.tex <==
\section{Discussion and conclusion}

\td{A bit boring discussion - what about more grand vision (integrated system, Odysseus project, GLA/TfL, policy makers using it etc) and also more technical future work/discussion items?}It is clear that there are benefits and drawbacks to all types of scans which are mostly dependent on the scientific use case. If the required output of the system is a \emph{single} region of space-time that engulfs surging sensors, then it is deemed that the PL scan is superior in terms of speed, simplicity and high spatial recall. If the user is not interested in a singular return region and requires a more visual heat map output of the domain, then the NET scan offers a much more localised view of the surge; boasting superior spatial precision. Indeed, the size of the region of interest also plays its part. The simplicity of the PL scan allows for much larger domains without increasing the run-time; for example, the whole city of London, UK. It was found that imposing a $16\times16$ grid on the entire London domain provided a sufficient resolution for detecting larger regions of increased activity -- shown in \cref{London Mapbox}, \cref{sec:more_discussion}. However, it is deemed that if data sources are confined to a network that sits in a relatively small region of space (e.g. a borough), then the NET scan is far superior in visualising localised hotspots with the added advantage of including the direction of the surged activity. For additional discussion see \cref{sec:more_discussion}.





